Aggregating Funnels for Faster Fetch&Add and Queues

Many concurrent algorithms require processes to perform fetch-and-add operations on a single memory location, which can be a hot spot of contention. We present a novel algorithm called Aggregating Funnels that reduces this contention by spreading the fetch-and-add operations across multiple memory locations. It aggregates fetch-and-add operations into batches so that the batch can be performed by a single hardware fetch-and-add instruction on one location and all operations in the batch can efficiently compute their results by performing a fetch-and-add instruction on a different location. We show experimentally that this approach achieves higher throughput than previous combining techniques, such as Combining Funnels, and is substantially more scalable than applying hardware fetch-and-add instructions on a single memory location. We show that replacing the fetch-and-add instructions in the fastest state-of-the-art concurrent queue by our Aggregating Funnels eliminates a bottleneck and greatly improves the queue's overall throughput.

==> pseudocode_agg.tex <==

\begin{algorithm*}
\begin{algorithmic}[1]
\Class{\Agg} \Comment{used to aggregate batches of \FetchAndAdd\ operations}
	\State int \x{value} \Comment{sum of values added at this \Agg}
%    \State int \x{sign} \Comment{$+1$ or $-1$ if \Agg\ handles positive or negative changes}
	\State Batch* \x{last} \Comment{last Batch in \Agg's list}
\EndClass	

\medskip

\Class{Batch} \Comment{represents a batch of operations on an \Agg}
	\State int \x{before} \Comment{\Agg's \x{value} before the batch}
	\State int \x{after} \Comment{\Agg's \x{value} after the batch}
	\State int \x{mainBefore} \Comment{value of \x{Main} before the batch}
	\State Batch* \x{previous} \Comment{pointer to previous Batch of operations on the \Agg}
\EndClass

\medskip

\State Shared variables:
\State int $\x{Main} \leftarrow 0$
\State \Agg* \x{Positive}$[0..m-1]$ \Comment{initially, for each \Agg\ $A$, $A.\x{value} = 0$ and
$A.\x{last}$ points to}
\State \Agg* \x{Negative}$[0..m-1]$ \Comment{a Batch with $\x{before}=\x{after}=\x{mainBefore}=0$ and $\x{previous}=\mbox{nil}$}

\medskip

\Function{int}{Fetch\&Add}{int \x{df}}
        \If{$\x{df} = 0$}
            \Return \op{Read}()\label{FAA0}
        \EndIf
        \State \Agg* $a \leftarrow $ \op{Choose\Agg}(\x{df}) \Comment{any \Agg\ in \x{Positive} or \x{Negative}, depending on sign of \x{df}}\label{chooseAgg}
	\State int $\x{aBefore} \leftarrow \FAA(a.\x{value}, \x{df})$\label{FAAagg}
	\State \textbf{wait until} $|a.\x{last}.\x{after}| \geq |\x{aBefore}|$ \Comment{spin until earlier operations on $a$ are done}\label{wait}	
    \State Batch* $\x{last} \leftarrow a.\x{last}$ \label{read-last}
    \If{$\x{last}.\x{after} = \x{aBefore}$}\Comment{operation is the first in a batch of operations}\label{delegatedTest}
		\State int $\x{aAfter} \leftarrow a.\x{value}$\Comment{get \Agg\ $a$'s \x{value} at the end of the batch of operations}\label{readValue}
		\State int $\x{mainBefore} \leftarrow \FAA(\x{Main}, \x{aAfter}-\x{aBefore})$\Comment{apply batch of operations on \x{Main}}\label{FAAMain}
		\State $a.\x{last} \leftarrow \mbox{new Batch}(\x{aBefore}, \x{aAfter}, \x{mainBefore}, \x{last})$\Comment{add Batch to $a$'s list}\label{newBatch}
		\State \Return{\x{mainBefore}}\label{return1}
	\Else \Comment{this operation is in a Batch already added to $a$'s list}
		\State Batch* $\x{batch} \leftarrow \x{last}$ \Comment{start from $a$'s last Batch}\label{search-begin}
		\While{$|\x{batch}.\x{before}| > |\x{aBefore}|$}\Comment{find batch with $|\x{batch}.\x{before}| \leq |\x{aBefore}| < |\x{batch}.\x{after}|$}\label{searchwhile}
			\State $\x{batch} \leftarrow \x{batch}.\x{previous}$
		\EndWhile\label{search-end}
		\State \Return $\x{batch}.\x{mainBefore} + \x{aBefore} - \x{batch}.\x{before}$\Comment{compute result to return}\label{return2}
	\EndIf
\EndFunction

\medskip

\Function{int}{Fetch\&AddDirect}{int \x{df}} \Comment{apply \FetchAndAdd\ directly to \x{Main}}
	\State \Return{\FAA(\x{Main}, \x{df})}\label{direct}
\EndFunction

\medskip

\Function{int}{Read(\hphantom{$\cdot$})}{} \Comment{read value directly from \x{Main}}
	\State \Return{\x{Main}}
\EndFunction

\medskip

\Function{int}{Compare\&Swap}{int \x{old}, int \x{new}}\Comment{any other available primitive can be applied similarly to \x{Main}}
	\State \Return{\op{CAS}(\x{Main}, \x{old}, \x{new})} \Comment{use hardware \op{CAS} directly on \x{Main}}
\EndFunction
%\Siddhartha{We need to modify this CAS to be an arbitrary Update(op, args) RMW operation}
\end{algorithmic}
\caption{Aggregating Funnel: a strongly linearizable Fetch\&Add implementation.\label{stump}
\Y{I suggest that we use either the variable $\textit{batch}$ or $\textit{last}$ but not both. My preference would be to use $\textit{batch}$.}}
\end{algorithm*}

\begin{algorithm}
\begin{algorithmic}[1]
\StartFromLine{35}
    \Function {\Agg *} {Choose\Agg} {int \x{df}}
        \State int $\x{g} \leftarrow \left\lfloor \x{threadIdx} / \sqrt{p} \right\rfloor $
        \If{$\x{df} > 0$}
            \Return $\x{Positive}[g]$
        \Else \xspace
            \Return $\x{Negative}[g]$
        \EndIf
\EndFunction
\end{algorithmic}
\caption{One possible implementation of the \op{Choose\Agg} function for $p$ threads using $m=\floor{\sqrt{p}}$ \Aggs\ for each sign.}\label{evenSpread}
\end{algorithm}






